Safe Reinforcement Learning Using Black-Box Reachability Analysis

Reinforcement learning (RL) is capable of sophisticated motion planning and control for robots in uncertain environments. However, state-of-the-art deep RL approaches typically lack safety guarantees, especially when the robot and environment models are unknown. To justify widespread deployment, robots must respect safety constraints without sacrificing performance. Thus, we propose a Black-box Reachability-based Safety Layer (BRSL) with three main components: (1) data-driven reachability analysis for a black-box robot model, (2) a trajectory rollout planner that predicts future actions and observations using an ensemble of neural networks trained online, and (3) a differentiable polytope collision check between the reachable set and obstacles that enables correcting unsafe actions. In simulation, BRSL outperforms other state-of-the-art safe RL methods on a Turtlebot 3, a quadrotor, a trajectory-tracking point mass, and a hexarotor in wind with an unsafe set adjacent to the area of highest reward.

==> Sections/A_implementation_details.tex <==
\section{Implementation Details}

\subsection{Data Collection and Processing}
\subsubsection{Data Collection}
The data was collected by letting the agent choose random actions in an empty environment in both cases for $500$ time steps. Then, this data was saved and used again while running the agents in both the training and testing environments.

\subsubsection{Data Processing and Warping}~
BRSL heavily depends on data-driven reachability analysis.
Getting the most suitable data that covers the whole space has a crucial effect on how conservative BRSL's forward reachability analysis is.
This conservatism worsens when we calculate the forward reachable sets for many timesteps; that is, each time step makes the reachable set zonotopes much larger.

To mitigate this problem, we apply a small trick to reduce the reachability zonotopes' volume.
First, we note that the state-space can be warped in the collected data such that an upper and a lower limit is imposed without loss of generality (WLOG).
We can enforce the position of a robot, for example, to be confined only within $[0, 1]$ WLOG.
In our examples, the robot's dynamics are position-invariant.
This means that we can confine the offline collected data to be within this range. 
We find empirically that this strategy significantly reduces BRSL's conservatism without impeding safety guarantees.
% For the Turtlebot example, 500 data points were more than enough to get our framework running. 

%\subsection{Environment Mimic}

%\subsubsection{Architecture}

%\subsubsection{Training}
%The loss function used for training is...



%\subsection{RTS Implementation}

%\subsubsection{Turtlebot}
%The Turtlebot's high-fidelity model is...

%We use the following planning model...


%\subsubsection{Quadrotor}
%The high-fidelity model is...

%The wind is modeled as...

%We use the following planning model...


\subsubsection{Approximating the Lipschitz Constant}

Determining a Lipschitz constant $L^\star$ and covering radius $\delta$ is, in general, difficult.
In this work, we apply the method from \cite[Remark 9]{alanwar2020data}.
Assume that the data $\statedata_-$ and $\actiondata$ (as in \eqref{eq:data}) are evenly distributed in $\statespace\times\actionspace$ (which are assumed to be compact).
Let $Z = (\statedata_-, \actiondata)$.
Then we approximate upper bounds for $L^\star$ and $\delta$ as
\begin{align}
    \hat{L}^\star &= \max_{\vc{z}_i, \vc{z}_j \in Z, j \neq i} \frac{\norm{\dyn(\vc{z}_i) - \dyn(\vc{z}_j)}_2}{\norm{\vc{z}_i - \vc{z}_j}_2},\ \regtext{and} \\
    \hat{\delta} &= \max_{\vc{z}_i \in Z} \min_{\vc{z}_j \in Z, j \neq i} \norm{\vc{z}_i - \vc{z}_j}_2,
\end{align}
where $\vc{z}_i \in Z$ is a minor abuse of notation to denote choosing $\vc{z}_i$ as a state/action pair from the data matrices in $Z$.



\subsection{Experiments}

\subsubsection{RL Agent Choice}
To select an RL agent for our experiments, we run a preliminary evaluation of three different agents for both robots: TD3 \cite{conf:TD3}, SAC \cite{conf:SAC}, and DDPG \cite{conf:DDPG}.
The agents are trained in randomized environments for $10^5$ time steps.
We choose TD3 for subsequent simulations as it outperforms SAC and DDPG in terms of maximum cumulative reward for both robots.


\subsubsection{Environment Mimic Sampling Details}
\TODO{explain how to do sampling from the stochastic model}



\subsubsection{Turtlebot Details}

The Turtlebot's control inputs are longitudinal and angular velocities.
Its maximum longitudinal velocity is $0.25$ m/s, and its angular velocity lies within $[-0.5, 0.5]$ rad/s.
The Turtlebot is equipped with wheel encoders and with a planar lidar that generates $18$ noisy distance measurements evenly spaced in a $180^\circ$ arc in front of the robot.
The Turtlebot requires a maximum of  $\nbrk = 3$ time steps to execute a failsafe braking maneuver, so we set $\nplan = 4$.


\subsubsection{Quadcopter Details}

The quadcopter control input at each time is a commanded velocity in each spatial direction.
The quadcopter's maximum speed is $5$ m/s (in any direction).
It is equipped with an IMU and a 16-channel lidar which generates noisy point cloud data in a $50^\circ$ vertical FOV and a $360^\circ$ horizontal FOV (a $360^\circ$-arc around the robot). 
The robot requires $\nbrk = 5$ time steps (i.e., 1 s at our discretization of 5 Hz) to come to a stop from its maximum speed, so we set $\nplan = 5$.


==> Sections/algorithms/alg_dream.tex <==
\begin{algorithm}[t]
\caption{Dreaming}
\label{alg:dream}
\KwInput{current RL agent state $\RLstate_k$, RL policy $\policy_\theta$, and environment mimic network $\mimic_\phi$}

\KwInOut{reward $\rewfunc$ and action $\action\brk$ per Assum. \ref{assumption:stop}}

$\dreamstate_k \leftarrow \RLstate_k$ // initialize dream state

\For{$j = k:(k+\nplan)$ \label{ln:dream1}}{
     $\mimicaction_j \leftarrow \policy_\theta(\dreamstate_j)$ // dream action \\ \label{ln:dream2}
     
     $\rew_j \leftarrow \rewfunc(\dreamstate_j,\mimicaction_j)$ // dream reward

     $\dreamstate_{j+1} \leftarrow \mimic_\phi(\dreamstate_{j+1},\mimicaction_j)$ // dream next state \\ \label{ln:dream3}
} \label{ln:dream4}

$\mimicaction_j \leftarrow \action\brk$ for all $j > k + \nplan$ // include failsafe \\

 \textbf{return} $\plan_k \leftarrow (\mimicaction_j)_{j=k}^\infty$ // dreamed plan
\end{algorithm}
